A Two-Layer Near-Optimal Strategy for Substation Constraint Management via Home Batteries

Within electrical distribution networks, substation constraints management requires that aggregated power demand from residential users is kept within suitable bounds. Efficiency of substation constraints management can be measured as the reduction of constraints violations w.r.t. unmanaged demand. Home batteries hold the promise of enabling efficient and user-oblivious substation constraints management. Centralized control of home batteries would achieve optimal efficiency. However, it is hardly acceptable by users, since service providers (e.g., utilities or aggregators) would directly control batteries at user premises. Unfortunately, devising efficient hierarchical control strategies, thus overcoming the above problem, is far from easy. We present a novel two-layer control strategy for home batteries that avoids direct control of home devices by the service provider and at the same time yields near-optimal substation constraints management efficiency. Our simulation results on field data from 62 households in Denmark show that the substation constraints management efficiency achieved with our approach is at least 82% of the one obtained with a theoretical optimal centralized strategy.

==> architecture/architecture.tex <==
In our proposed framework, 
each house $u \in U$ is provided with a battery (and related circuitry/inverters). This allows us to implement demand shifts via charge/discharge commands to such batteries (see, e.g.,~\cite{ZLH20}). This also allows us to easily apply our methodology to most houses, given the widespread availability and low costs of modern home batteries ({\em applicability}). As we want a fully automatic framework, we need \hl{software} computing such charge/discharge commands. However, this cannot be done at the \Ac{DSO} premises, as having the utility directly acting on batteries at user premises would not be acceptable for users. Furthermore, commands for batteries need to be computed \hl{at} a high rate (e.g., every 5 minutes) and to be reliably delivered. To this aim, using Internet links may entail delays or even missed communication, whilst using new dedicated communication lines would be too expensive.

%
  In order to solve such issues, we organize our framework as a {\em two-layer} architecture named \Ac{DALB} (see \cref{fig:ebr_arch}). Namely,
%
layer 1 is a centralized software service called \Ac{DAPP}~\cite{TSG17_DAPP}. One instance of \Ac{DAPP} has to be run {\em for each substation}, with a periodicity of one day. This entails that \Ac{DAPP} instances are run at the \Ac{DSO} premises, possibly using powerful workstations. The main goal of \Ac{DAPP} is to acquire power demands from all \hl{houses} and compute individualized power bounds $P_u^{low}, P_u^{high}$ for the next day. 
  If all houses $u \in U$ are able to keep their resulting demand $e_u(t)$ inside the bounds $[P_u^{low}(t), P_u^{high}(t)]$ for all $t \in T_s$, then the aggregated power outside of  the desired substation power profile $\Delta(e)$ is minimized.
  Note that power bounds $P_u^{low}, P_u^{high}$ may be sent via the Internet to each house $u$, as such communication takes place only once a day and may be delayed.
  Finally, we note that \Ac{DAPP} uses coarse-grained time slots (i.e., one hour).
%
  Layer 2 is a decentralized software called \Ac{EBR}. One instance of \Ac{EBR} must be run {\em on each house} $u \in U$. 
  This entails that \Ac{EBR} must be run on \hl{inexpensive low-resources hardware} (a Raspberry Pi in our experiments).
  The main goal of \Ac{EBR} is to acquire the current power demand and \Ac{SOC} of the battery in house $u$,
and to compute the charge/discharge actions for the battery itself. 
Such actions will modify the home demand $e_u(t) = d_u(t) + a_u(t)$, by either increasing it ({\em charge} action $a_u(t) > 0$, e.g., from 7 to \hl{8 AM} in \cref{fig:ebr_example} (right)) or decreasing it ({\em discharge} action $a_u(t) < 0$, e.g., from 8 to \hl{9 AM} in \cref{fig:ebr_example} (right)). The objective is to minimize the power outside the bounds $[P_u^{low}(t), P_u^{high}(t)]$ provided by the \Ac{DAPP} service\hl{, without compressing or increasing the user demand in the full period}.
Furthermore, if an \Ac{PEV} is also present, then \Ac{EBR} may also be used to drive the \Ac{PEV} charge/discharge (thus employing the so-called \Acs{V2H}). 
Note that:
\begin{enumerate*}

\item The battery is always plugged-in and ready to accept charge/discharge commands. On the contrary, the \Ac{PEV} is plugged-in only when the residential user decides to do so.

\item There are no restrictions, other than the physical ones (e.g., do not exceed the maximum power rate), on battery usage. On the contrary, the \Ac{PEV}, once plugged-in, must be fully charged within a given deadline.

\item Both battery and \Ac{PEV} must be equipped with a \Ac{BEM}~\cite{battery_management.book,HKLYGHL16,CKPAE18,KFJBH18}, accepting (wireless) commands to: 1) read the current \Ac{SOC}; 2) charge/discharge the battery/\Ac{PEV}. In this latter case, the \Ac{BEM} receives a software signal $a \in \Reals$, and the battery/\Ac{PEV} is charged (if $a \geq 0$) or discharged (otherwise) 
  with $a$ kW rate
until the next signal $a'$ is received.

\end{enumerate*}


==> conclusions/conclusions.tex <==

\newbox\anyboxname
\sbox\anyboxname{\Acl{DAPP}}

In this paper, we presented \Acl{DALB}, a two-layer computing service \hl{that} is able to enforce aggregated power demand constraints on \Acl{EDN} substations. \Acl{DALB} is composed of two services, both based on the \Acl{MPC} methodology: \hl{\mbox{\Acl{DAPP}}}, operating once a day at the substation level and at utility premises, and \Acl{EBR} (also employing a novel {\em adaptive} \Acl{MPC}), operating once every 5 minutes at user premises on hardware with limited computational resources.
More in detail, such services act as a hierarchical controller: \hl{\mbox{\Acl{DAPP}}} sets up the long-term goal for \Acl{EBR}, which directly controls local home batteries via charge/discharge commands \hl{to} meet such goals. Users privacy is also preserved, as only their overall demand is sent to the \Acl{DSO}, as it already happens with home mains, and home batteries are not actuated by the \Acl{DSO}.

Using power demands recorded in 62 houses in Denmark
by the EU
project SmartHG~\cite{Alim2015}, we experimentally showed that \Acl{DALB} is able to reduce aggregated demand bounds violations w.r.t. the unmanaged demand by about 50\% on average (w.r.t. 61\% reduction obtained by \hl{a} theoretical optimal centralized solution). This is achieved while meeting real-time requirements on the available hardware, both at the substation and at the houses level.

Our \Acl{DALB} framework currently focuses on satisfying the substation (feeder) power bounds. As future work, we plan to investigate how to extend it to enforce other network-level restrictions, e.g., on power flow.


==> intro/intro.tex <==
In an \Ac{EDN}, many electrical substations provide electricity to the residential users connected to such substations. On each substation $s$, one of the main goals for a \Ac{DSO}  is \Ac{SCM}, that is, enforcing suitable desired lower and upper bounds on the aggregated power demand resulting from the houses connected to $s$. In fact, \Ac{SCM} enables savings for the \Ac{DSO}, e.g., in substations maintenance and energy peak production~\cite{URAHT18}. 
%
In the context of smart grids, computational services may be used %by the aggregator
to enforce {\em efficient} and {\em effective} \Ac{SCM}. %to the \Ac{DSO}.
Namely, efficiency is measured as the reduction of bounds violations w.r.t. the unmanaged aggregated power demand, i.e., the complement to 1 of the time average of the ratio between managed w.r.t. unmanaged demand outside bounds. On the other hand, \Ac{SCM} is effective if it minimizes user discomfort and is technically %and economically
viable.
The main obstacles for efficient and effective computational services for  \Ac{SCM} are the following:
\begin{enumerate*}
\item using \Ac{DR}, i.e., relying on residential users to autonomously respond to price incentives, is often ineffective, as users tend to ignore price signals~\cite{TSG17_DAPP};
\item using \Ac{DLC}, i.e., active power curtailment and reactive power control, is ineffective as well, as it may lead to a loss of useful energy~\cite{DFBS2018}.
\end{enumerate*}
A promising way of achieving efficient and effective \Ac{SCM} is to install low-cost batteries at each user premises, and then automatically controlling them. In this way, bounds violations can be reduced by automatically shifting user demand, which also minimizes user discomfort. Although centralized control of such batteries would achieve optimal efficiency, it faces the following main obstacles:
\begin{enumerate*}
\item reliability of communication lines, as every few minutes a command for each home battery must be sent to each user (we note that, typically, home electricity mains can transmit, but not receive);
\item above all, for security and privacy reasons, many users would not accept such a centralized solution, as a service provider (e.g., a utility or an aggregator) is demanded of controlling the storage at the user premises. 
\end{enumerate*}
Thus, we have to rely on hierarchical control strategies for home batteries. 



{\bf Related work.} Many single-layer\hl{,} as well as hierarchical methodologies\hl{,} have been proposed in the context of smart grids, with different goals.
As for single-layers methodologies,
in~\cite{TSG17_DAPP,MMMSTGHPE18}
individualized \Ac{IBR} and \Ac{ToU} price policies  for residential houses connected to a substation $s$  are investigated, \hl{to} perform peak shaving.
In~\cite{JSK18} a 
data analytical \Ac{DR} management scheme for residential load
is proposed \hl{to} reduce the peak
load demand.
In~\cite{EHB21},\hl{ }a privacy-aware stochastic multiobjective optimization framework that considers
the objectives of both consumers and utility companies
in a\hl{n} \Ac{DR} scheme.
Unfortunately, users tend to ignore price signals~\cite{TSG17_DAPP}. This motivates the goal of this paper, i.e., automatically shifting user demand. 

A single-layer approach involving \Ac{DLC} of \Ac{HVAC} appliances is proposed in~\cite{ETPC19}. Unfortunately, demanding \Ac{DSO} of controlling devices at user premises is hardly accepted by users. Furthermore, here we focus on  actuating home batteries.
In~\cite{ZWHL20}, a methodology is presented to allow a storage aggregator to invest and operate a central physical storage unit, by virtualizing it into separable virtual capacities and selling it to users. 
In~\cite{DL20}, an intelligent multi-microgrid energy management method is proposed based on artificial intelligence techniques, \hl{to} protect user privacy. In our setting, we only use the information from user mains, which is already available to \Acp{DSO}. % and aggregators.
In~\cite{ZLH20}, a 
methodology for optimal residential battery operation in a single house is proposed, \hl{to} minimize electricity costs. 
Finally, the approaches in~\cite{ZZCKLSG21,CKM20} 
focus on \hl{the} scheduling of \Acp{PEV} only.
However, in our setting\hl{,} we are interested in \Ac{SCM}, which is not addressed in~\cite{DL20,ZWHL20,ZLH20,ZZCKLSG21,CKM20}.

The methodologies described above mainly rely on \hl{the} charge/discharge of home batteries \hl{to} perform power demand shifting. Many other methodologies (see, e.g.,~\cite{SXZ14,JBBSKN20} and citations thereof) have also been proposed which rely on scheduling appliances usage, to be either automatically or manually applied. However, such approaches require either modern smart appliances, which may not be available in many houses, or rely on users manually applying the scheduling, which is ineffective~\cite{TSG17_DAPP}. In our setting, we focus on batteries as they allow both 1) \hl{more} widespread applicability, as it is simpler, especially in non-modern houses, to install a home battery than many smart appliances, and 2) to always rely on a completely automatic approach.

As for hierarchical methodologies, in~\cite{SYEAAM19} a hierarchical distributed \Ac{MPC} approach is presented to solve the energy management problem in the multitime frame and multilayer optimization strategy.
In~\cite{LCSP18} a hierarchical day-ahead \Ac{DSM} model is
proposed, where renewable energy sources are integrated.
In~\cite{CGWLZ20} a hierarchical approach is presented for distributed voltage optimization in high-voltage and medium-voltage \Acp{EDN}.
In~\cite{WXWHGLST20} a two-layer distributed cooperative control method for islanded networked microgrid systems is described.
In~\cite{BFATM20} an optimal multiobjective control \hl{methodology} is discussed for power flow regulation and compensation of reactive power and unbalance in AC microgrids.
In~\cite{RBSPR18} a bilevel optimization framework is presented \hl{to} minimize energy cost for commercial building \Ac{HVAC} systems.
In~\cite{SXCG15} a distributed energy management strategy
for the optimal operation of microgrids is described.
In~\cite{DST19} a distributed consensus-based approach is proposed to solve the grid welfare
problem by deriving an real-time pricing scheme that facilitates an automated \Ac{DR}.
problem by deriving \hl{a} real-time pricing scheme that facilitates an automated \Ac{DR}.
In~\cite{TBS11} a hierarchical \Ac{MPC} of smart grid systems is described \hl{to} balance demand and supply.
Such methodologies cannot be applied to our setting, as they do not address the problem of constraining the aggregated demand of residential users within given desired bounds.
In~\cite{PMNH20}, a two-layer control framework is proposed \hl{to} perform peak shaving (i.e., keeping the aggregated power demand below a given upper threshold). However, in our setting, we are interested in acting on domestic batteries, which allows a more widespread use, while~\cite{PMNH20} focuses on (smart) \Ac{HVAC} \hl{only}. 

Finally, ``adaptive'' \Ac{MPC} often refers to techniques able to automatically adjust, at run-time, the model parameters~\cite{TLPE18}, e.g., the weights of some constraints (see~\cite{AdaptiveBook15} and citations thereof). 
In~\cite{SF17}, a lightweight \Ac{MPC} scheme able to adjust its prediction horizon has been presented and evaluated on a simple industrial process plant. However, in~\cite{SF17} horizon changes are driven by the need of tuning the reference trajectory of the model. 
Instead, in our work, we vary the horizon so as to keep the house inside given power bounds.

Summing up, \hl{to} achieve efficient and effective \Ac{SCM}, we need a framework \hl{that} avoids centralized solutions (typically not accepted by users for privacy and security reasons) and \hl{rely} neither on user autonomously changing their habits nor in (possibly expensive) smart appliances.

\begin{figure}
  \IncludeGraphics[width=0.5\textwidth]{../architecture/figs/DAPP-LEHMS.png}
  \caption{The proposed architecture
  }\label{fig:ebr_arch}\label{fig:ebr_overall}
  \end{figure}

{\bf Main Contributions.} To overcome the obstructions described above, in this paper we propose a novel hierarchical two-layer computational service for efficient and effective \Ac{SCM}. We call such a service  \Acl{DALB} (\Acs{DALB}, see \cref{fig:ebr_overall}). 
In the following, we list the main contributions of our approach.

\begin{enumerate}[wide]

\item \Acs{DALB} encloses two services, each running at different levels of the \Ac{EDN} (substations and houses) and with different periodicity (orders of days w.r.t. orders of minutes).

\begin{itemize}[wide]

\newbox\anyboxname
\sbox\anyboxname{ \Ac{DAPP}}

\item
The first layer is the 
\hl{\mbox{\usebox\anyboxname}}
service (based on~\cite{TSG17_DAPP}), which is executed independently for each \Ac{EDN} substation $s$. The \Ac{DAPP} goal is to maintain the aggregated power demand of $s$ within \hl{the} desired range given in input, by computing individualized and time-dependent lower and upper bounds on the power demand of each house connected to $s$. The duration of such bounds must be long enough to allow users to actually shift their power demand
(one day in our experiments).

\item
The second layer is the \Ac{EBR} service, which must be run independently on each residential user $u$. The \Ac{EBR} goal is to maintain the demand of $u$ within the power bounds decided for $u$ by \Ac{DAPP}. Namely, \Ac{EBR} acts as a \Ac{HEMS} which is able to control \hl{the} charge and discharge of home batteries, thus shifting the demand of $u$ to stay inside the given power bounds. To this aim, \Ac{EBR} must compute actions on home batteries with a sufficiently short periodicity (5 minutes in our experiments), \hl{to} catch up with variations in the demand of $u$.

\end{itemize}

\item \Acs{DALB} may be either directly employed by the \Ac{DSO} itself or offered by a \Ac{DSRA}. In this latter case, the \Ac{DSO} provides the \Ac{DSRA} with the desired bounds on the aggregated demand of $s$ and will pay the \Ac{DSRA} so that violations on such bounds are minimized. In the following, we will refer to the entity running \Acs{DALB} as {\em \Acs{DALB} provider}.
\item \Ac{DAPP} only requires in input the bounds on the substation (always provided by the \Ac{DSO}) and the residential user power demand (already provided by the electricity main in each house), thus it is executed at the \Acs{DALB} provider premises, possibly using powerful computing devices. On the other hand,  \Ac{EBR} is responsible to actuate charge/discharge of home batteries with real-time requirements, thus it is executed at each user premises. \hl{Communication} between the two services takes place when \Ac{DAPP} sends to \Ac{EBR} the lower and upper bounds for the given user power demand: this happens only once a day without real-time constraints, thus it can \hl{rely}, e.g., on a typical home Internet connection.
\item Running \Ac{EBR} at each user premises entails that an inexpensive and small microcomputer with limited computational resources, i.e., small RAM and low CPU frequency (in our experiments, we used a Raspberry Pi), can be used. 
\item Both \Ac{DAPP} and \Ac{EBR} are based on the \Ac{MPC} methodology~\cite{chen-etal:2013:tsg,LKZQF16}. That is, with the given periodicity (1 day and 5 minutes, respectively), \Ac{DAPP} and \Ac{EBR} solve a suitable optimization problem 
which, depending on forecasts for the user power demand, minimizes the power outside the given bounds. From the solution to the optimization problem, \Ac{DAPP} extracts the bounds for each user, while \Ac{EBR} extracts the charge/discharge actions for batteries.
%
The main parameter for the \Ac{MPC} methodology is the {\em receding horizon} used for the optimization problem, i.e., how many hours in the future must be considered. While \Ac{DAPP} receding horizon is typically one day (as it is standard in the day-ahead energy market), for real-time-constrained \Ac{EBR} it should be experimentally estimated in an initialization phase, which may be costly. 
To this aim, for each user, the detailed power demand on a past period (e.g., one year)
is needed, which may be unavailable. Furthermore, 
such initialization could not catch up with modifications in user power demand habits, which would diminish \Ac{EBR} effectiveness. \Ac{EBR} solves such a problem by employing an {\em adaptive} algorithm, which automatically adjusts, at run-time, the receding horizon. Moreover, \Ac{EBR} succeeds in doing this without violating real-time requirements. To the best of our knowledge, this is the first time that such an algorithm is presented.

\end{enumerate}


{\bf Experimental Results.} We experimentally evaluate the efficiency and effectiveness of  \Acs{DALB} using data \hl{collected} from sensors in 62 Danish households connected to the same substation during the SmartHG project~\cite{Alim2015}. 
As a result:
%
\begin{enumerate*}

\item \Acs{DALB} is able to achieve a 50\% efficiency (i.e., reduction of substation bounds violations w.r.t. the unmanaged demand). This is a near-optimal solution, as a {\em theoretical} optimal centralized approach on the same scenario would achieve 61\% efficiency, i.e., our solution is 82\% as effective as the theoretical optimal one. 
We remark that the results obtained in the centralized version of our approach cannot be actually achieved in our setting for the previously explained reasons (i.e., lack of reliability of communication lines and users security and privacy reasons).

\item \Ac{EBR} can be run on a Raspberry Pi, meeting the required hard-real-time deadlines. As for \Ac{DAPP}, it may easily be run by a desktop computer. 


\end{enumerate*}


==> methodology/methodology.tex <==
In this section, we describe our \Ac{DALB} service, by giving details of 
\Ac{DAPP} and \Ac{EBR} (for a high-level view, see \cref{fig:ebr_overall}). In the following, for both services, we will distinguish between {\em configuration input} and {\em online input}. That is, configuration input must be given once and for all when starting a service for the first time, while online input needs to be periodically acquired. 


{\bf \Acs{DAPP} Input and Output.}
The main configuration input consists of the following:
%
  \begin{enumerate*}

  \item Duration $\tau_l \in \RealsGZ$, in minutes, of the power limits \hl{output from} \Ac{DAPP}.

  \item Period $\tau_s \in \RealsGZ$, in minutes, of \Ac{DAPP} invocations (i.e., \Ac{DAPP} computes output power limits every $\tau_s$ minutes). Note that time slots duration $\tau_l$ must divide $\tau_s$. This also defines the horizon length $H_s = \frac{\tau_s}{\tau_l}$ of the \Ac{MPC} methodology used by \Ac{DAPP}.

  \item For each house $u \in U$, battery maximum capacity $Q_{u,E}$ (in kWh) and battery maximum and minimum power rates $M_{u, E}$ and $m_{u, E}$, in kW (see, e.g.,~\cite{TSG17_DAPP,ZLH20}).

    \item For each house $u \in U$, minimum and maximum power demand (in kW) $C_u^{low}, C_u^{high} \in \RealsGZ$, as from the electricity contract.



  \end{enumerate*}
  

\hl{The} online input consists of the following:
%
\begin{enumerate*}

\item (Ordered) set $T_s = \{t_1, \ldots, t_{H_s}\}$ of the future time slots, \hl{each} lasting $\tau_l$ minutes. 
\item Desired 
bounds for the substation $s$ to which houses in $U$ are connected $P_{s}^{low}, P_{s}^{high} : T_s \to \Reals$ (in kW).

  \item For each house $u \in U$, power demand $\tilde{d}_u$ (in kW), as the difference between consumption (from appliances and \Ac{PEV}) and production (from \Aclp{PVP}), taken at intervals at least
  $\tau_l$. 
  This is used to compute \hl{$d_u : T_s \to \Reals$ (in kW) as} power demand forecasted for the next period $T_s$.
    Here we are interested in computing the forecast in negligible time, thus, for a given time slot $t$, the forecast is computed by a %simple
    discounted average on the demands in the same time slot $t$ in the past days (in our experiments, we consider 10 days in the past).
    For an %complete
    overview of demand forecasting methods, see~\cite{YMH17,LWZ20}. Note that, as \Ac{DAPP} cannot directly drive \Acp{PEV}, the power used on each house to recharge the \Ac{PEV} is included in $d_u$.


  \end{enumerate*}

Finally, \hl{the} \Ac{DAPP} \hl{output consists}, for each house $u \in U$, of two power profiles $P^{low}_u, P^{high}_u : T_s \to \Reals$. \hl{Such power profiles will be given as input to} \Ac{EBR}. \hl{Namely} \Ac{EBR},  executed at $u$ premises, will have to keep the resulting power demand $e_u$ inside $[P^{low}_u(t), P^{high}_u(t)]$ as most as possible, for all time slots $t$. If each \Ac{EBR} running on each house $u \in U$ succeeds in this task, then the overall aggregated power outside the desired substation bounds $\Delta(e)$ 
will be minimized.

{\bf \Acs{EBR} Input and Output.}  
In the following, we focus on a given house $u \in U$, thus we will assume index $u$ to be understood.
The main configuration input of \Ac{EBR} consists \hl{of}:
%
  \begin{enumerate*}

  \item The starting horizon length $H_i \in \Naturals$ and horizon length changing step $H_\delta \in \Naturals$ used for the \Ac{AMPC} methodology employed by \Ac{EBR}. 

  \item The period $\tau \in \RealsGZ$, in minutes, of \Ac{EBR} invocations (i.e., \Ac{EBR} decides an action every $\tau$ minutes). We also require \Ac{PEV} and battery actions to be computed within $\zeta$ minutes. This allows \Ac{EBR} to correctly assume that computed actions will be held for $\tau - \zeta$ minutes. Namely, if $\zeta$ is sufficiently low, computed actions will be actually held by \Ac{PEV} and battery for almost $\tau$ minutes.

  \item 
  \Ac{PEV} maximum capacity $Q_P$ (in kWh) and \Ac{PEV} maximum and minimum power rates $M_P$ and $m_P$ (in kW). 
  Furthermore, battery and \Ac{PEV} efficiency for charge $\alpha_E, \alpha_P$ and discharge $\beta_E, \beta_P$, respectively.

  \end{enumerate*}
  

On the other hand, the online input consists of the following:
%
\begin{enumerate*}

\item The (ordered) set $T = \{t_1, \ldots, t_H\}$ of the future time slots. 
  All time slots except 
  \hl{$t_1$} last $\tau_l$ minutes, i.e., the frequency of changes in power limits. 
  Duration of $t_1$ is defined so as $t_2$ starts at a multiple of $\tau_l$. E.g., if power limits change every hour ($\tau_l = 60$) and the current time-stamp is 10:15, $t_1$ will last 45 minutes.

  \item The power limits for $u$ \hl{as an output from} \Ac{DAPP}.

  \item Power demand $\tilde{d}$ currently being requested to the grid (excluding \Ac{PEV}, which is managed separately). Using the same techniques of \Ac{DAPP}, the forecast for the demand $d : T \to \Reals$ on the next $H$ periods of $\tau_l$ minutes is computed.

\item Current state of charge for both the battery $\tilde{Q}_E$ and the \Ac{PEV} $\tilde{Q}_P$ (\hl{$\tilde{Q}_P = -1$} if it is currently not plugged-in).

  \item If $\tilde{Q}_P \neq -1$, the deadline for \Ac{PEV} recharging ${\cal D}_P \in \Naturals$, s.t. ${\cal D}_P = i \geq 0$ iff the \Ac{PEV} must be completely recharged in at most $i$ \hl{minutes}. 
    We assume that the residential user manually specifies the deadline for the complete \Ac{PEV} recharge when plugging the \Ac{PEV}.

  \end{enumerate*}

Finally, \hl{the} \Ac{EBR} \hl{output consists} of \hl{commands} $a_E, a_P \in \Reals$. Namely, $a_E$ is the charge (if $a_E \geq 0$) or discharge ($a_E < 0$) command, in kW, for the battery in the current time \hl{slot}. 
Analogously, if the \Ac{PEV} is plugged-in (i.e., if $\tilde{Q}_P \geq 0$) then $a_P$ is the charge/discharge command for the \Ac{PEV}. 




  \begin{figure}
  \begin{tabular}{p{0.7\columnwidth}p{0.7\columnwidth}}
  \begin{minipage}{0.7\columnwidth}
  \IncludeGraphics[width=1.05\textwidth]{figs/adapt_code.pdf}
  \end{minipage}
  &
  \hspace*{-2.5cm}\begin{minipage}{0.7\columnwidth}
  \IncludeGraphics[width=1.05\textwidth]{figs/lahems_code.pdf}
  \end{minipage}
  \\
  \end{tabular}
  \vspace*{-0.3cm}
  \caption{Simplified control-flow diagram for \Acs{DAPP} (left) and \Acs{EBR} (right), \hl{also showing the main variables used}}\label{fig:adapt_lahems_code}
  \end{figure}

{\bf \Acs{DAPP} Base Algorithm.}
\hl{Both} \Ac{DAPP} \hl{and} \Ac{EBR} \hl{algorithms are based on the} \Ac{MPC} \hl{methodology. As for the system model (e.g., batteries and power demand) as well as for the underlining} \Ac{MPC} \hl{scheme, we follow well-established approaches from the literature, e.g.,}~\cite{TSG17_DAPP,ZLH20}. 
Every $\tau_s$ minutes, \hl{the} %main
\Ac{DAPP} algorithm computes the power limits for all houses $u \in U$. To this aim, a \Ac{LP} problem $L_1$ (designed by suitably extending~\cite{TSG17_DAPP}) with receding horizon $H_s$ for layer 1 is generated and solved.
Namely, $L_1$ contains $6|U||T_s| + 3|T_s| + |U|$ constraints, defined over $4|U||T_s| + |U| + 2|T_s|$ real-valued variables, which are detailed in the following. 

\vspace*{-.5cm}
\begin{equation}\label{ess_b}
\forall u \in U, t \in T_s. \; b_{u, E}(t + 1) = b_{u, E}(t) + \frac{\tau_l}{60}a_{u, E}(t)
\end{equation}

\vspace*{-.1cm}
Constraint~\eqref{ess_b} states that the \Ac{SOC} $b_{u, E}(t + 1)$ (in kWh) of the battery in house $u$ at a given time slot $t + 1$ is the result of applying action $a_{u, E}(t)$ (in kW) to \Ac{SOC} $b_{u, E}(t)$ at the previous time slot $t$, also considering time slot duration in minutes $\tau_l$.

\vspace*{-.3cm}
\begin{equation}\label{ess_b_s_e}
\forall u \in U. \; b_{u, E}(t_1) = b_{u, E}(t_{|T_s|} + 1) = \frac{Q_{u, E}}{2}
\end{equation}

Constraint~\eqref{ess_b_s_e} states that the behavior of the battery must be cyclic, i.e., the starting and ending \Ac{SOC} of the battery (within time slots set $T_s$, which lasts one day in our experiments) in a given house $u$ must be both half of the battery maximum capacity $Q_{u, E}$. In this way, there are no preferences among different executions of \Ac{DAPP} in different days. 

\vspace*{-.5cm}
\begin{equation}\label{inside_pp_up}%\label{inside_pp_down}
\forall u \in U, t \in T_s. \;P_{u}^{low}(t) \leq a_{u, E}(t) + d_u(t) \leq P_{u}^{high}(t)
\end{equation}

Constraint~\eqref{inside_pp_up} states that the {\em collaborative power profile} for each $u \in U$ must always be inside the bounds $P^{low}_u, P^{high}_u$ to be output for user $u$. Note that, following the nomenclature in~\cite{TSG17_DAPP}, ``collaborative power profile'' does not refer to collaborations between users, but to the fact that each user is willing to follow the price policies decided by \Ac{DSO} using \Ac{DAPP}. Namely, such collaborative power profile is defined by applying an action on the battery $a_{u, E}(t)$ to the current demand $d_u(t)$, thus obtaining $a_{u, E}(t) + d_u(t)$.

\vspace*{-.3cm}
\begin{equation}\label{b_bounds}
\forall u \in U, t \in T_s. \;0 \leq b_{u, E}(t) \leq Q_{u, E}
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{a_bounds}
\forall u \in U, t \in T_s. \;m_{u, E} \leq a_{u, E}(t) \leq M_{u, E}
\end{equation}

Constraints~\eqref{b_bounds} and~\eqref{a_bounds} require that the power demand shift $a_{u, E}$ for user $u$ is within the limits of user $u$ {\em flexibility}, i.e., within the power rate and capacity of the battery in house $u$ (also Constraint~\eqref{ess_b} is involved, as it defines the future \Ac{SOC}).

\vspace*{-.5cm}
\begin{equation}\label{pp_bounds}
\forall u \in U, t \in T_s.\; C^{low}_u \leq P_{u}^{low}(t) \leq  P_{u}^{high}(t) \leq C^{high}_u
\end{equation}

Constraint~\eqref{pp_bounds} requires that the output bounds $P^{low}_u, P^{high}_u$ for user $u$ must be within the electricity contract of $u$.

\vspace*{-.2cm}
\begin{equation}\label{d_bounds}
\forall t \in T_s.\; \Delta^{high}(t)\geq 0, \Delta^{low}(t)\geq 0
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{outside_subs_up}
\forall t \in T_s.\; \sum_{u \in U}P_{u}^{high}(t) \leq P_{s}^{high}(t) + \Delta^{high}(t)
\end{equation}
\vspace*{-0.2cm}
\begin{equation}\label{outside_subs_down}
\forall t \in T_s.\; \sum_{u \in U}P_{u}^{low}(t) \geq P_{s}^{low}(t) - \Delta^{low}(t)
\end{equation}

Constraints~\eqref{d_bounds}--\eqref{outside_subs_down} define the worst-case aggregated powers $\Delta^{high}$ exceeding $P_s^{high}$ and $\Delta^{low}$ going below $P_s^{low}$. The objective function of $L_1$ is to minimize all such aggregated power exceeding substation bounds, i.e., $\sum_{t \in T_s}\Delta^{high}(t) + \sum_{t \in T_s}\Delta^{low}(t)$.

  


\hl{Finally, every $\tau_s$ minutes, the} \Ac{DAPP} \hl{output values} for power limits $P^{low}_u(t), P^{high}_u(t)$, for all $u \in U, t \in T_s$,
are computed by solving, every $\tau_s$ minutes, the \Ac{LP} problem $L_1$ via a \Ac{LP} solver and then extracting, from the obtained solution, the values for decision variables $P^{low}_u(t), P^{high}_u(t)$ (the corresponding control-flow diagram is shown in \hl{the} left part of \cref{fig:adapt_lahems_code}).




{\bf \Acs{EBR} Base Algorithm.}  In each house $u \in U$, every $\tau$ minutes, the main \Ac{EBR} algorithm computes charge/discharge decisions on battery and/or \Ac{PEV}, basing on the battery and/or \Ac{PEV} current \Ac{SOC}, on the current household power demand, on forecasted future power demand, and on the known future power limits $P^{low}_u, P^{high}_u$ from \Ac{DAPP}. 
  In order to compute the charge/discharge commands, a \Ac{MILP} problem $L_2$ with receding horizon $H$ for layer 2 is generated and solved.
  $L_2$ consists of two separate sets $L_{2E}, L_{2P}$ of constraints. Constraints in $L_{2E}$ 
  deal with fixed battery dynamics and
  thus are always present. Constraints in $L_{2P}$ 
  are defined only when the \Ac{PEV} is plugged-in. We have that $L_{2E}$ is defined by $22H + 2$ constraints on $5H + 1$ continuous decision variables and $4H$ binary decision variables. On the other hand, $L_{2P}$ is defined by at most $6H + 2$ constraints on at most $3H$ continuous decision variables and $H$ binary decision variables, depending on $|T_P|$, being $T_P$ the subset of time slots in $T$
  in which the \Ac{PEV} will stay plugged-in. 
  In the following, we describe such constraints in more detail. We recall that we focus on a given house $u \in U$, thus we will assume index $u$ to be understood.

\vspace*{-.5cm}
\begin{equation}\label{energy_balance}
\forall t \in T. e(t)\!=\!d(t) + a_E^{ch}(t) - \beta_E a_E^{dis}(t) 
+\eta(t)(a_P^{ch}(t) - \beta_Pa_P^{dis}(t))
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{e_constr}
\forall t \in T. \; C^{low} \leq e(t) \leq C^{high}
\end{equation}

Constraint~\eqref{energy_balance} defines the power $e(t)$ requested or generated by the house in time slot $t \in T$ as the sum of all houses power consumption (power demand $d(t)$, charge commands for battery and \Ac{PEV} $a_E^{ch}(t), a_P^{ch}(t)$) and power production (discharge commands for battery and \Ac{PEV} $a_E^{dis}(t), a_P^{dis}(t)$). All such values are in kW. Battery and \Ac{PEV} discharge commands also take into account round-trip inefficiencies $0 < \beta_E,\beta_P < 1$.  Constant $\eta(t)$ is defined, for a given time slot $t$, as the fraction of $t$ in which the \Ac{PEV} is plugged-in. 
Constraint~\eqref{e_constr} requires such resulting power demand $e(t)$ to be inside the ranges of the household electricity contract. 

\vspace*{-.3cm}
\begin{equation}\label{ess.start}
b_E(t_1) = \tilde{Q}_E, 0 \leq b_E(t_H + 1) \leq Q_E
\end{equation}
\vspace*{-0.7cm}
\begin{equation}\label{ess_dyn}
\forall t \in T. \; b_E(t + 1) = b_E(t) + \frac{|t|}{60} (\alpha_E a_E^{ch}(t) - a_E^{dis}(t))
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{ess_dyn_bool2}
\forall t \in T. \; y_E(t) \to a_E^{ch}(t) = 0, \neg y_E(t) \to a_E^{dis}(t) = 0
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{ess_bounds}
\forall t \in T. \; 0 \leq b_E(t) \leq Q_E, 0 \leq a_E^{ch}(t) \leq M_E, 0 \leq a_E^{dis}(t) \leq m_E
\end{equation}

Constraints~\eqref{ess.start} and~\eqref{ess_dyn} define the behavior of the battery, i.e., the starting \Ac{SOC} $\tilde{Q}_E$  (in kWh) is read from sensors, and the \Ac{SOC} at time $t + 1$ is obtained by adding to the \Ac{SOC} at time $t$ the action taken at time slot $t$, multiplied by the time slot duration $|t|$.
In case of a charge action, the efficiency coefficient $0 < \alpha_E < 1$ is also considered. Constraint~\eqref{ess_dyn_bool2} allows us to distinguish between a charge and a discharge action, which is required \hl{to} apply the known battery efficiencies $\alpha_E, \beta_E$. Furthermore, the battery physical constraints on power rate and capacity are taken into account by Constraint~\eqref{ess_bounds}.
Note that the Constraints~\eqref{ess_dyn_bool2} \hl{are} {\em guarded constraints} of the form $\gamma \to L({\cal X}) \leq K$ or $\neg \gamma \to L({\cal X}) \leq K$, where $L$ is a linear function, ${\cal X}$ is a set of bounded variables (i.e., all variables in ${\cal X}$ are defined on a suitable bounded interval), $\gamma$ is a binary variable not in ${\cal X}$ and $K$ is a constant. Since all our decision variables are bounded, such constraints are translated into linear constraints as follows: $\gamma \to L({\cal X}) \leq K $ is equivalent to $(\sup(L({\cal X})) - K)\gamma + L({\cal X}) \leq \sup(L({\cal X}))$, while $\neg \gamma \to L({\cal X}) \leq K$ is equivalent to $(K - \sup(L({\cal X})))\gamma + L({\cal X}) \leq K$. In such formulas, $\sup(L({\cal X}))$ may be easily computed as $L$ is linear and all variables in ${\cal X}$ are bounded~\cite{TSG17_DAPP}.


\vspace*{-0.3cm}
\begin{equation}\label{pev.start}
b_P(t_1) = \tilde{Q}_P
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{pev_dyn}
\forall t \in T_P. \; b_P(t + 1) = b_P(t) + \eta(t)\frac{|t|}{60} (\alpha_P a_P^{ch}(t) - a_P^{dis}(t))
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{pev_dyn_bool2}
\forall t \in T_P. \; y_P(t) \to a_P^{ch}(t) = 0, \neg y_P(t) \to a_P^{dis}(t) = 0
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{pev_bounds}
\forall t \in T_P. \; 0 \leq b_P(t) \leq Q_P, 0 \leq a_P^{ch}(t) \leq M_P, 0 \leq a_P^{dis}(t) \leq m_P
\end{equation}

Constraints~\eqref{pev.start}--\eqref{pev_bounds} define the analogous behavior for the \Ac{PEV}. Note that such constraints are defined on the set $T_P = \{t_1, \ldots, \tilde{t}\}$ of the time slots in which the \Ac{PEV} is actually plugged-in. This implies that Constraints~\eqref{pev.start}--\eqref{pev_bounds} are only present when the \Ac{PEV} is currently plugged-in, thus they are in $L_{2, P}$. Note that the Constraints~\eqref{pev_dyn_bool2} are guarded constraints (see above).

\begin{equation}\label{pev_final2}
b_P(\tilde{t} + 1) = \min\{Q_P, \tilde{Q}_P + \alpha_PM_P{\cal D}_P\}\min\left\{1, \frac{\sum_{t \in T}|t|}{{\cal D}_P}\right\}
\end{equation}


  To define the goal for \Ac{PEV} recharging, 
  we have to consider two aspects, both handled by Constraint~\eqref{pev_final2} in $L_{2, P}$. On the one hand, the input deadline specified by the user for the \Ac{PEV} complete recharge may be infeasible w.r.t. the current \Ac{SOC} (e.g., it is infeasible to completely recharge the \Ac{PEV} from 0 kWh in 1 hour). In order to avoid 
  $L_2$ to turn out infeasible only because of this, \Ac{EBR} first computes the \Ac{SOC} attainable with the currently specified deadline, i.e., $\tilde{Q}_P + \alpha_PM_P{\cal D}_P$.
  On the other hand, the \Ac{PEV} may be expected to be unplugged at time slot $\tilde{t}$ within the current time horizon, or in a time slot \hl{that} will be considered in a future \Ac{MILP}. In the former case, the \Ac{PEV} must be completely charged at $\tilde{t}$. 
  In the latter case, we require the final charge of the \Ac{PEV} to be proportional to the remaining time before unplugging the \Ac{PEV}, i.e., $\frac{\sum_{t \in T}|t|}{{\cal D}_P}$. 

\vspace*{-0.2cm}
\begin{equation}\label{inside_pplus1}
\forall t \in T. \; y^{high}(t) \to e(t) \leq P^{high}(t)
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{inside_pplus2}
\forall t \in T. \; \neg y^{high}(t) \to e(t) \geq P^{high}(t)
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{inside_pminus1}
\forall t \in T. \; y^{low}(t) \to e(t) \geq P^{low}(t)
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{inside_pminus2}
\forall t \in T. \; \neg y^{low}(t) \to e(t) \leq P^{low}(t)
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{zplus_ok1}
\forall t \in T. \;y^{in}(t) \to y^{high}(t) + y^{low}(t) \geq 2
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{zplus_ok2}
\forall t \in T. \;\neg y^{in}(t) \to y^{high}(t) + y^{low}(t) \leq 1
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{z_def1}
\forall t \in T. \; y^{in}(t) \to z(t) = 0
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{z_def2}
\forall t \in T. \; \neg y^{high}(t) \to z(t) = e(t) - P^{high}(t)
\end{equation}
\vspace*{-0.5cm}
\begin{equation}\label{z_def3}
\forall t \in T. \; \neg y^{low}(t) \to z(t) = -e(t) + P^{low}(t)
\end{equation}
\vspace*{-0.8cm}
\begin{equation}\label{zp_constr}
\forall t \in T. \; 0 \leq z(t) \leq \max\{P^{low}(t) -C^{low}, C^{high} - P^{high}(t)\}
\end{equation}

The objective function of $L_2$ \hl{minimizes} the power outside the limits decided by \Ac{DAPP} for the given house. To this aim, such exceeding power in time slot $t \in T$ is modeled by variable $z(t)$ (having bounds as in Constraint~\eqref{zp_constr}), thus the objective function to be minimized is $\sum_{t \in T}z(t)$. By using guarded constraints (see above), the decision variables $z(t)$ are defined by:

\begin{itemize}
\item   Constraints~\eqref{inside_pplus1} and~\eqref{inside_pplus2}, where binary variable $y^{high}(t)$ is set to true iff the resulting power $e(t)$ exceeds the upper bound $P^{high}(t)$;
\item   Constraints~\eqref{inside_pminus1} and~\eqref{inside_pminus2}, where binary variable $y^{low}(t)$ is set to true iff the resulting power $e(t)$ is below the lower bound $P^{low}(t)$;
\item Constraints~\eqref{zplus_ok1} and~\eqref{zplus_ok2}, where binary variable $y^{in}(t)$ is set to true iff the resulting power $e(t)$ is inside the bounds interval $[P^{low}(t), P^{high}(t)]$;
\item Constraints~\eqref{z_def1}--\eqref{z_def3}, where, exploiting the binary variables defined in Constraints~\eqref{inside_pplus1}--\eqref{zplus_ok2}, the real variable $z(t)$ is defined to be 0 iff $e(t) \in [P^{low}(t), P^{high}(t)]$, and to be the power outside the bounds interval $[P^{low}(t), P^{high}(t)]$ otherwise.
\end{itemize}




\sloppy


\hl{Finally, every $\tau$ minutes, the} \Ac{EBR} \hl{output values} for
battery and/or \Ac{PEV} charging/discharging actions
are computed by \hl{solving the} \Ac{MILP} problem $L_2$ via a \Ac{MILP} solver and then extracting, from the obtained solution, the actions  for the first time slot in $T$. If $L$ \hl{is} infeasible, then a default action is selected, which is designed to minimize user discomfort. That is, if the \Ac{PEV} is not currently plugged-in or is already fully charged, then no action is taken, i.e., $(a_E, a_P) = (0, 0)$. Otherwise, the \Ac{PEV} is charged as much as possible, also discharging the battery as much as possible, \hl{i.e., $a_P = \min\{M_P, \frac{Q_P - \tilde{Q}_P}{\tau}, C^{high} - d(t_1) + $ $\beta_E\min\{m_E, \frac{Q_E - \tilde{Q}_E}{\tau}\}\}, a_E = -\min\{m_E, \frac{Q_E - \tilde{Q}_E}{\tau}, \frac{a_P}{\beta_E}\}$. Instead, if $L$ is feasible, then, for $x \in \{E, P\}$, $a_x = a^{ch}_x(t_1)$ if $a^{ch}_x(t_1) \geq 0$, and $a_x = a^{dis}_x(t_1)$ otherwise.}
The corresponding control-flow diagram is shown in \hl{the} right part of \cref{fig:adapt_lahems_code}.

\fussy

{\bf \Acs{EBR} Adaptive Algorithm.}  Our adaptive algorithm is based on the fact that using a high value for the horizon $H$ does not imply that we obtain better exceeding power minimization. This is due to: i) uncertainties stemming from power demand forecasting, which are worse for higher values of the horizon, and ii) higher computation time typically required to solve \Acp{MILP} with higher horizons, as the number of both constraints and decision variables linearly depends on $H$. Thus, our adaptive algorithm works as follows. Instead of setting up only one \Ac{MILP} $L$ with fixed receding horizon $H$, as it is done in the literature, \Ac{EBR} sets up and separately solves 3 different \Acp{MILP} with receding horizon $h \in \{H, H - H_\delta, H + H_\delta\}$ respectively. For each of such \Acp{MILP}, \Ac{EBR} maintains the current objective function value $\hat{c}(h)$ (i.e., by accumulating the values of the \Ac{MILP} objective functions as computed by the \Ac{MILP} solver). When, for some $h \neq H$, the value for $h$ is better than the value for the current horizon $H$,
i.e., $\hat{c}(h) < \hat{c}(H)$,
the current horizon $H$ 
is updated to $h$ and all objective function values $\hat{c}(h)$ are reset to 0. Note that only the actions computed with the current horizon $H$ (which are computed first) are sent to batteries actuators. Namely, \Ac{MILP} problems with other horizons are only used to automatically adjust the current horizon, so that the exceeding power is further minimized.

In order to meet real-time requirements, \Ac{EBR} uses a twofold strategy. First of all, \Ac{EBR} stops \Ac{MILP} solver execution if it exceeds  $\zeta$ minutes. In this case, the current \Ac{MILP} problem $L$ is handled as if it were infeasible (i.e., minimizing user discomfort). This entails that battery actions are \hl{held} for $\tau -  \zeta$ minutes. Since, for small values of $\zeta$,  $\tau - \zeta \approx \tau$, this is in agreement with \Ac{MILP} constraints
which assume computed actions for battery and \Ac{PEV} to be held for all current time slot duration $\tau$. 
Second, after having computed the actions for battery and \Ac{PEV}, \Ac{EBR} would be idle till the end of the current time slot duration $\tau$ (neglecting periodic tasks such as downloading new power limits or reading the current power demand). \Ac{EBR} exploits such although idle time to compute the actions with horizons $H - H_\delta, H + H_\delta$, thus achieving horizon adjustment without overhead. 




==> problem_form/problem_form.tex <==
\begin{figure*}
  \begin{subfigure}{0.45\textwidth}
    \IncludeGraphics[scale=0.5]{figs/example_p_0_25.pdf}
  \end{subfigure}
~
  \begin{subfigure}{0.45\textwidth}
    \IncludeGraphics[scale=0.5]{figs/example_home_p_0_25.pdf}
  \end{subfigure}
  \caption{Input and output for layer~1 (left) and layer~2 (right) in the most demanding day of our experiments (2014-01-29, see \cref{sec:exps_setup}). Left figure shows aggregated power demand before (``historical'') and after (``\Acs{DALB} resulting'') applying \Acs{DALB},
    %on all houses,
    right figure shows power demand
    of the most demanding house before (``historical'') and after (``\Acs{EBR} resulting'') applying \Acs{EBR} on that house  }\label{fig:ebr_example}\label{fig:dapp_example}
  \end{figure*}


In our setting, 
a set of residential houses $U$ are connected to the same substation $s$. 
The \Ac{DSO} $D$ is able to compute, basing on documentation and recorded power demand data, {\em desired power bounds} for the substation $P_{s}^{low}(t), P_{s}^{high}(t)$ (in kW) for suitable time slots $t \in T_s$ (in our experiments, each $t$ lasts one hour and all $t \in T_s$ refer to the next day). Let $d_u(t)$ be the power requested to the grid by house $u \in U$ in time slot $t \in T_s$, and let $d(t) = \sum_{u \in U} d_u(t)$ be the {\em aggregated} power demand in $t$ (in kW). Furthermore, let $\Delta(d, t) = \Delta^{low}(d, t) + \Delta^{high}(d, t) = \max\{P_{s}^{low}(t) - d(t), 0\} + \max\{d(t) - P_{s}^{high}(t), 0\}$ be the power (in kW) outside $P_{s}^{low}(t), P_{s}^{high}(t)$, if any, when the aggregated demand is $d$. If $D$ is able to keep the overall aggregated power outside the desired substation bounds $\Delta(d) = \sum_{t \in T_s}\Delta(d, t)$ as low as possible, then it will
save in substation maintenance and energy peak production~\cite{URAHT18}.
%
Given this, we want to devise a software framework \hl{to} {\em shift} power demand $d_u$ of each $u \in U$, so as to obtain a power demand $e = \sum_{u \in U} e_u = \sum_{u \in U} d_u + a_u$ s.t. the aggregated power outside bounds $\Delta(e)$
  is minimized over a long-enough period (e.g., one year). 
%
We want such a framework 
to have the following properties:
\begin{enumerate*}
\item It must be {\em completely automatic}, by shifting each household power demand {\em without} involving residential user direct actions, \hl{to} minimize user discomfort. 
  Note that demand shifting must not entail power curtailment~\cite{DFBS2018}.
\item It must be {\em easily applicable} to most houses, with as low hardware installations as possible.
\item It must be {\em technically viable}. That is, the aggregated demand which results from the power shifts must \hl{reduce} the peaks outside the substation desired bounds. 
  Moreover, we have to show that real-time requirements arising from the hardware-software interaction are \hl{met}. 
\end{enumerate*}
\cref{fig:dapp_example} (left) shows an example of our problem formulation, in which we only consider the upper bound on the substation 
by using input and output 
selected from the most demanding day in our experiments (see \cref{sec:exps_setup}). Note that shifts may be positive (e.g., from \hl{0 AM} to \hl{5 AM}, where the resulting demand green curve is above the historical demand blue curve) as well as negative (e.g., from \hl{8 AM} to 11 AM). In the day depicted in \cref{fig:dapp_example}, 
the reduction is about 50\%, measured as $1 - \frac{\Delta(e)}{\Delta(d)}$. 

 \input{architecture/architecture.tex}


==> related_work/related_work.tex <==
%To the best of our knowledge, there are no previous works presented in the literature which aim to address the peak shaving and load balancing problems for \Acp{EDN} with a two-layer strategy similar to the one we propose here. In the following, we will discuss separately the previous contributions to each of our layers, i.e., the distribution level and the domestic level. We finally discuss other related multi-layers approaches.

%{\bf Load balancing and peak shaving.}
The \Ac{DAPP} service proposed here is based on the DAPP service described in~\cite{TSG17_DAPP}. However, the DAPP service in~\cite{TSG17_DAPP} can only be used for peak shaving, whereas here we are also interested in load balancing. Furthermore, in~\cite{TSG17_DAPP} the bounds computed for each house are proposed to residential users via individualised {\em price policies}, without \Acp{HEMS} enforcing. This entails that complementary approaches to actually check possible deviations from desired user behaviours are needed~\cite{Hayes2014sgcomm,MMMSTGHPE18}.

In~\cite{PMNH20}, a two-layer control framework is proposed in order to perform peak shaving. However, in our case we cannot use the methodology presented in~\cite{PMNH20} because, in order to minimise additional hardware installation, here we are interested in acting on domestic \Acp{ESS}, whilst in~\cite{PMNH20} only (smart) air conditioners and water heaters are considered. Furthermore, we are also interested in load balancing, which is not addressed in~\cite{PMNH20}. Finally, here we are also interested in assessing real-time requirements and computational resources feasibility, %for local (i.e., at the residential level) computation,
which is not addressed in~\cite{PMNH20}. A single-tier approach involving \Ac{DLC} of \Ac{HVAC} appliances is proposed in~\cite{ETPC19}, with similar limitations in our setting. Hierarchical methodologies have also been proposed with different goals than load balancing and peak shaving: as an example, in~\cite{CGWLZ20} a hierarchical approach is presented for distributed voltage optimisation if high-voltage and medium-voltage \Acp{EDN}, and in~\cite{WXWHGLST20} a two-layer distributed cooperative control method for islanded networked microgrid systems is described.

In~\cite{PEPBC16}, a single-layer control framework, involving \Acp{PEV} and \Acp{ESS}, is proposed to minimise energy procurement cost in a neighbourhood of smart households. In our setting, we cannot rely on~\cite{PEPBC16} since we are interested in a two-layer framework, in order to minimise communication between \Ac{DSO} and residential users. Furthermore, we are interested in load balancing and peak shaving by setting bounds at the substation level, which is not allowed by~\cite{PEPBC16}.

In~\cite{ZWHL20}, a methodology is presented to allow a storage aggregator to invest and operate a central physical storage unit, by virtualising it into separable virtual capacities and selling to users. In our setting, instead, an aggregator collects a residential house neighbourhood in order to provide services to a \Ac{DSO}.

In~\cite{DL20}, an intelligent multi-microgrid energy management method is proposed based on artificial intelligence techniques, in order to protect users privacy. In our setting, we only use the information from user mains, which is already available to \Acp{DSO} and aggregators.

In~\cite{ZLH20}, a %non-\Ac{MPC}
methodology for optimal residential battery operation in a single house is proposed, in order to minimise electricity costs. This is similar to the \Ac{EBR} service proposed here. However, here we are interested in enforcing power bounds decided by the \Ac{DSO}, which cannot be done with the methodology in~\cite{ZLH20}. The same limitations hold for the methodologies in~\cite{LKRD20,EPMBC15,CZC16,LRDLBAC17}.

Finally, we point out that, in the literature, ``adaptive'' \Ac{MPC} mostly refers to a set of techniques able to automatically adjust, at run-time, the model parameters~\cite{TLPE18}, such as, e.g., weights of some constraints (see~\cite{AdaptiveBook15} and citations thereof). Typically, such algorithms are not designed to be run on limited-resource hardware, which is our focus here. Moreover, in our setting we do not need to adjust model parameters. %, as our experimental results will show.
In~\cite{SF17}, a lightweight \Ac{MPC} scheme able to adjust its prediction horizon has been presented and evaluated on a simple industrial process plant. However, horizon changes are driven by the need of tuning the reference trajectory of the model w.r.t. the plant time delays and inverse response. Instead, in this work we are interested in varying the horizon so as to maximise the saving for the user.

%% %\begin{Section}[sec:adaptive_rel_w]{Adaptive \Ac{MPC} schemas}
  
%% {\bf Adaptive \Acs{MPC} schemas.} In the literature, ``adaptive'' \Ac{MPC} mostly refers to a set of techniques able to automatically adjust, at run-time, the model parameters~\cite{TLPE18}, such as, e.g., weights of some constraints (see~\cite{AdaptiveBook15} and citations thereof). Typically, such algorithms are not designed to be run on limited-resource hardware, which is our focus here. Moreover, in our setting we do not need to adjust model parameters. %, as our experimental results will show.

%% In~\cite{SF17}, a lightweight \Ac{MPC} scheme able to adjust its prediction horizon has been presented and evaluated on a simple industrial process plant. However, horizon changes are driven by the need of tuning the reference trajectory of the model w.r.t. the plant time delays and inverse response. Instead, in this work we are interested in varying the horizon so as to maximise the saving for the user.

%% %\end{Section}
%% %Many works have

%% %\begin{Section}[sec:hems_ctrl]{Control of \Acsp{HEMS}}
%% {\bf Control of \Acsp{HEMS}.} Research has
%% been presented in the literature in order to help residential users in following a given price policy (see~\cite{TSG17_DAPP} and citations thereof), so that their electricity bill is minimised, or %directly
%% to help \Acp{DSO} and/or retailers by acting at the household level. In the following, we categorise such works on their high-level organisation: {\em distributed} or {\em centralised}. %the type of the service they offer.

%% %\begin{Section}[sec:rw_dec_control_batt_pev]{Control of \Acs{ESS} and \Acs{PEV}}

%% %% {\bf Distributed Control of \Acs{ESS} and \Acs{PEV}}.
%% %% This category focuses on services which %directly
%% %% control and actuate an \Acs{ESS} and/or a \Acs{PEV}.
%% We first focus on services which %directly
%% control and actuate an \Ac{ESS} and/or a \Ac{PEV}.
%% Hence, the papers in such category are the closest to our paper. %The most important contributions in this category are the following.

%% In~\cite{EPMBC15}, a collaborative evaluation of
%% dynamic-pricing and peak power limiting-based \Ac{DR} strategies
%% with a bi-directional utilisation possibility for \Ac{PEV} and \Ac{ESS} is realised. A \Ac{HEMS} structure is provided for this purpose.
%% %% A
%% %% distributed small-scale renewable energy generation system, the
%% %% \Acs{V2H} and \Acs{V2G} capabilities of a \Acs{PEV} together with two-way energy
%% %% trading of \Acs{ESS}, and different \Acs{DR} strategies are all combined in
%% %% a single \Acs{HEMS} for the first time in the literature.
%% The differences between the present paper and~\cite{EPMBC15} are the following:
%% \begin{enumerate*}%[wide]
%% %% \item %in order
%% %% to minimise user discomfort, \Acs{EBR} has the goal of fully recharge the \Acs{PEV}, whilst in~\cite{EPMBC15} a fixed lower bound is provided;
%% %% \item \Acs{EBR} cost function also considers CO$_2$ emissions and energy distribution (not present in~\cite{EPMBC15}); %and does not explicitly provide a hierarchy on energy selling (as it is done in~\cite{EPMBC15});
%% \item \Ac{EBR} is based on an adaptive algorithm, while~\cite{EPMBC15} does not consider adaptiveness;
%% \item evaluation of \Ac{EBR} economic viability also considers additional hardware and installation costs, not covered in~\cite{EPMBC15};
%% \item \Ac{EBR} has also been technically evaluated in both a laboratory microgrid and on %limited
%% resource-constrained
%% hardware, while results in~\cite{EPMBC15} were obtained by simulation on a Desktop computer;
%% \item \Ac{EBR} is designed so as to provide secure software updates, while~\cite{EPMBC15} does not consider security issues;
%% \item our experimental results are based on 62 households %and 186
%% \Ac{PEV} measurements, also considering different scenarios of \Ac{ESS} and \Ac{PEV} usage, whereas only 1 household with 1 \Ac{PEV} is considered in~\cite{EPMBC15}.
%% \end{enumerate*}

%% In~\cite{CZC16} a
%% simple effective online algorithm is presented for the charging and discharging decisions of \Ac{ESS} that minimises the electricity cost
%% in the presence of electricity price fluctuations and renewable
%% energy supplies, without relying on the future information of
%% prices, demands, or renewable energy supplies. In~\cite{LRDLBAC17}
%% a comprehensive methodology is presented to optimally control lead-acid batteries operating under dynamic pricing schemes in both
%% independent and aggregated ways, taking into account the effects
%% of the charge controller operation, the variable efficiency of the
%% power converter, and the maximum capacity of the electricity
%% network. In~\cite{mishra-etal:2012:e-energy}, the authors explore how to
%% lower electricity bills without requiring consumer involvement
%% using an intelligent battery charging system, called SmartCharge,
%% and an on-site battery array to store low-cost energy for use
%% during high-cost periods. The approaches in~\cite{CZC16,LRDLBAC17,mishra-etal:2012:e-energy} cannot be used in our context as they do not handle \Acp{PEV}, which, differently from other \Acp{ESS}, can be not always available (i.e., they are available only when plugged-in) and need to be recharged at a given deadline. %, and they are not guaranteed to work with limited hardware computational resources.

%% %% \begin{Section*}[sec:rw_cent_control_batt_pev]{Centralised Control of \Ac{ESS} and \Ac{PEV}}

%% %{\bf Centralised Control of \Ac{ESS} and \Ac{PEV}}.
%% For the sake of completeness, we also discuss 
%% %This category focuses on
%% substation-level or \Ac{EDN}-level services, which handle multiple \Acp{ESS} and \Acp{PEV} on different houses in a coordinated way. % the most important and recent works which target \Ac{ESS} and \Ac{PEV}, but in a centralised and coordinated way.
%% %% rather than in a decentralised and independent way as it is our focus here. The most important contributions in this category are the following.

%% In~\cite{WZB19}, a %dissipativity based distributed economic
%% model predictive control approach is developed for the operation of battery energy storage networks in residential microgrids.
%% In~\cite{SSK16}, an effective approach is proposed for
%% %% decreasing the losses
%% %% payment
%% increasing the efficiency and reliability of \Ac{EDN} operation,
%% %% also considering the uncertainties of electricity prices in
%% %% a day ahead energy market
%% by
%% using \Acp{ESS}
%% and demand response. In~\cite{SDL16}, 
%% a real-time centralised power balancing solution is proposed,
%% taking into account the uncertainty of the renewable generation, loads, and electricity prices and aiming at minimising the long-term system cost.
%% In~\cite{PP19}, a sequential procedure is presented for short term operation of an aggregator to minimise the cost of the consumer and risk of the aggregator.
%% Finally, many papers in the literature are dedicated to the problem of controlling large populations of \Acp{PEV}, e.g., see~\cite{TW17,SWWDW16}. %Here, instead, our focus is in minimising energy bills for residential houses in a decentralised way.

%% With respect to such works, our contributions may be summarised as follows.
%% \begin{enumerate*}%[wide]
%% \item In this paper, the \Ac{DR} approach is taken, which is best accepted by residential users because of privacy and security issues~\cite{advanced.web}. As an example, in works coordinating \Acp{PEV} charging, it is necessary for a residential user to let the \Ac{DSO}/retailer to know when the \Ac{PEV} needs to be charged.
%% \item In the papers outlined above, it is {\em necessary} that \Acp{DSO}/retailers coordinate installation and running of the computational service used. In this paper, it is possible for a single residential user to use \Ac{EBR}, without any need of coordination with other users.
%% %\item  CO2 is never taken into account
%% %\item  PEV readiness is rarely taken into account
%% %\item actual economic evaluation is missing
%% \end{enumerate*}




%% %% \end{Section*}


%% %\begin{Section*}[sec:rw_dec_appl]{Control of Selected Appliances}

%% %% {\bf Control of Selected Appliances}.
%% %% This category focuses on services which control selected appliances (e.g., \Acs{PEV}, washers, driers), acting on a single household.
%% %% Such schedules may be actuated autonomously if the appliances are ``smart''. Otherwise, schedules must be manually applied by residential users.
%% %% %The most important and recent
%% %% Good examples of state-of-the-art
%% %% contributions in this category are the following.

%% %% %% In~\cite{WZWWZW15}, a robust-index method is proposed to tackle the challenges of uncertainties caused by customer behaviour in order to
%% %% %% minimise comfort violation in household load scheduling.
%% %% In~\cite{RL16}, the authors classify various appliances into five sets considering their different
%% %% energy consumption and operation characteristics, and provide
%% %% an electricity load scheduling algorithm in order to maximise the overall
%% %% net utility of a residence while satisfying its budget limit. In~\cite{MCSL16}, the authors introduce a novel concept
%% %% of cost efficiency-based residential load scheduling framework
%% %% to improve the economic efficiency of the residential electricity consumption.
%% %% %% The cost efficiency is defined as the ratio of
%% %% %% consumer total consumption benefit to its total electricity pay-
%% %% %% ment during a certain period. We develop a cost-efficient load
%% %% %% scheduling algorithm for the demand-side day-ahead bidding
%% %% %% process and real-time pricing mechanism by using a fractional
%% %% %% programming approach.
%% %% In~\cite{ZLSON16}, a learning-based
%% %% demand response strategy is developed for regulateable loads with
%% %% a special focus on home heating, ventilation, and air conditioning.
%% %% In~\cite{BSMG17}, an autonomous
%% %% electrical energy management-based cost reduction solution is proposed for peak load
%% %% times using a \Acs{HEMS}.
%% %% %% Within
%% %% %% a home environment, both the real time and the schedulable
%% %% %% appliances are connected with smart meter through \Acs{HEMS}.
%% %% Finally, some works in the literature propose methods which control or schedule selected appliances in a centralised way (see, e.g.,~\cite{PEPBC16} and citations thereof).


%% %% The \Acs{EBR} service we introduce here may be considered as complementary to such works, as they both shift loads, but in different ways. Nevertheless, \Acs{EBR} has the following advantages w.r.t. the above listed papers. %w.r.t. scheduling of single appliances:
%% %% \begin{enumerate*}%[wide]
%% %% \item \Acs{EBR} also works with \mbox{non-smart} appliances, non-specified appliances and non-automated appliances.
%% %% %\item Schedules are typically computed for long periods (e.g., one day), and may not be able to react to changes in the house demand. On the other hand, \Acs{EBR} may ``correct'' previous decisions after 5 minutes, if necessary.
%% %% \item \Acs{EBR} only needs to configure the batteries and/or the \Acs{PEV}. On the other hand, the approaches listed above require a separate configuration for each type of appliance.
%% %% %the configuration phase is much more complicated in the papers listed above, as each type of appliance has to be configured separately. %On the other hand, \Acs{EBR} only needs to configure the battery and/or the \Acs{PEV}.
%% %% \item The residential user may be almost unaware of \Acs{EBR} running in the background, the only input required being the deadline for \Acs{PEV} recharging. On the contrary, with the approaches discussed above, in order to schedule single appliances, more inputs are needed from the user (e.g., time for washer, lighting, etc.).
%% %% %\item When scheduling multiple appliances, there are multiple possible failures. On the other hand, \Acs{EBR} only has to control two appliances at most (batteries and/or \Acs{PEV}).
%% %% %\item When scheduling multiple appliances, the service has to read the status and the demand of each appliance. On the other hand, \Acs{EBR} only needs to read the overall power demand of all appliances. This makes \Acs{EBR} more robust to failures.
%% %% \end{enumerate*}

%% %\end{Section}


==> results/exps_res.tex <==

  Given the experimental setting described in \cref{sec:exps_setup}, in this section we show our 
  experimental results. 
  Namely, in \cref{all-box:fig} we present, for each \Ac{KPI} of \Ac{EBR} (see \cref{eval_kpi.tab}), the corresponding statistics as Box-and-Whiskers plots~\cite{tukey1977}. \hl{Since} each \Ac{KPI} is measured for every house, the plots in \cref{all-box:fig} provide, for each \Ac{KPI}, the statistics (i.e., average, interquartile range, outliers) on all houses. Furthermore, \cref{exps_res.tab} shows the results for the overall evaluation of the \Ac{DALB} service.
  In the following, we discuss the results \hl{of} the given \Acp{KPI}.

  \begin{figure*}
  \vspace*{-0.7cm}
  \begin{subfigure}{0.33\textwidth}
  \IncludeGraphics[width=\textwidth]{figs/AvgSolTime.png}
    \vspace*{-1.cm}
  \caption{\Acl{AMST}
  }
  \label{fig:mst_avg}
  \end{subfigure}
  ~
  \begin{subfigure}{0.33\textwidth}
  \IncludeGraphics[width=\textwidth]{figs/MissDeadl.png}
    \vspace*{-1.cm}
  \caption{\Acl{MMD}
  }
  \label{fig:mmd}
  \end{subfigure}
  ~
  \begin{subfigure}{0.33\textwidth}
  \IncludeGraphics[width=\textwidth]{figs/HorChange.png}
    \vspace*{-1.cm}
  \caption{\Acl{NHC}
  }
  \label{fig:nhc}
  \end{subfigure}
  \vspace*{0.7cm}
  \caption{Box-and-Whisker plots~\cite{tukey1977} for the main \Acsp{KPI} of \Acs{EBR}. In each plot, the box boundaries are the farthest points that are not outliers (i.e., that are within 1.5 the interquartile range), the line inside the box is the statistical median, and the circles are data more than 1.5 times the interquartile range from the end of a box.}\label{all-box:fig}
  \end{figure*}



\textbf{Demand Outside Bounds Reduction and Users Discomfort}. The main result of our \Ac{DALB} service consists in the fact that we \hl{achieve} a high reduction on the peaks outside substation desired bounds, without user \hl{discomfort.} \cref{exps_res.tab} shows that the demand peaks outside the substation desired bounds (considering both demands higher than the upper bound and lower than the lower bound) are halved in all our experimental scenarios. This is achieved with a \Ac{MPDF} equal to $0$ in all houses, i.e., deadlines for \Ac{PEV} recharging are never missed. Furthermore, the theoretical optimal reduction achieved in ideal conditions by the \Ac{DAPP} collaborative profile computed in a centralised way 
is about 60\% in all scenarios,
thus our near-optimal approach is at least 82\% as efficient as the theoretical optimal one. 

We remark that these results have been achieved by using the same inexpensive hardware that would have been needed by a non-\Ac{MPC}-based strategy. 
For the sake of comparison, consider a simple strategy where there is only one layer, consisting in a computational service acting on each house. The input of such service, call it \Ac{SDALB}, is the same as \Ac{EBR}, but instead of the power bounds computed by \Ac{DAPP}, \Ac{SDALB} is directly fed with the desired substation bounds $P_s^{low}, P_s^{high}$ and the number of houses $|U|$. Given this, \Ac{SDALB} first computes the house power bounds as $\frac{P_s^{low}}{|U|}, \frac{P_s^{high}}{|U|}$. Then, \Ac{SDALB} computes battery and \Ac{PEV} actions in a greedy way, i.e., the battery is charged (within its physical limits) when the current
demand is below the upper bound $\frac{P_s^{high}}{|U|}$, and discharged otherwise. Such a simple strategy, while requiring the same hardware as \Ac{DALB}, 
achieves a reduction of
substation constraint management violation of about 38\%, compared to 50\%
obtained with our approach.




  \textbf{Computation Time}. We recall that \Ac{EBR} is designed \hl{to} compute each battery and/or \Ac{PEV} action in at most  $\zeta = 30$  seconds. First of all, we point out that \Ac{MILP} deadlines violations are very few, as shown in  \cref{fig:mmd}. Namely, \cref{fig:mmd} shows that, for most houses, at most 5\% (and 2\% on average) of all \Ac{MILP} problems solved require more than 30 seconds to be solved, thus missing the real-time deadline. Furthermore, also considering statistical outliers, the percentage of missed deadlines is always below 13\% in all houses.
  On the other hand, \cref{fig:mst_avg} 
  shows that most \Ac{MILP} solver invocations, on average, require much lower computation time than 30 seconds. Namely, for most houses, the average of the times needed to solve all \Ac{MILP} problems (given there is one \Ac{MILP} solved every 5 minutes over one year, such average is computed on about 105,000 values on each house) turns out to be between 1 and 3 seconds in all scenarios. Furthermore, also considering the statistical outliers, for all houses the average \Ac{MILP} solving time is at most 5 seconds.
  Such results show that \Ac{EBR} is indeed
  a lightweight application as required and fully meets the requirements for real-time computation on the target low-resource device (Raspberry  Pi).
  Finally, as for \Ac{DAPP} computation time, it typically requires at most 1 second, which is negligible w.r.t. \Ac{DAPP} periodicity (1 day). This is not surprising, as the \Ac{MILP} problems defined in \Ac{DAPP} are actually \Ac{LP} problems (i.e., they do not involve binary decision variables).




\textbf{Adaptive Algorithm Effectiveness}. In order to show the effectiveness of the adaptive algorithm employed by \Ac{EBR}, 
\cref{fig:nhc} shows the results for the \Ac{NHC} \Ac{KPI} (see \cref{eval_kpi.tab}). Namely, in all scenarios and all houses, there are 4 horizon changes every 1000 \Ac{MILP} solver invocations on average. 
This shows that our adaptive algorithm is 
effective, as it is able to adapt to very different conditions, depending on the scenario and \hl{the} current home behaviour.



    \begin{table}
    \vspace*{.5cm}
      \centering
      \caption{Results for \Acs{DALB} evaluation}\label{exps_res.tab}
      
      \begin{tabular}{L{0.02\textwidth}L{0.11\textwidth}L{0.11\textwidth}L{0.14\textwidth}}
        \toprule
        \textbf{$s$} & \textbf{\Acs{LADOBR}} & \textbf{\Acs{DADOBR}} & \textbf{$\frac{\Acs{LADOBR}}{\Acs{DADOBR}}$}
        \\\hline
        0 & 0.5 & 0.61 & 0.82\\\hline
        0.25 & 0.53 & 0.63 & 0.83\\\hline
        0.5 & 0.48 & 0.58 & 0.83\\\bottomrule
\end{tabular}
\vspace*{-0.3cm}
\end{table}



==> results/exps_setup.tex <==

    \begin{table*}
      \centering
      \caption{List of \Acsp{KPI} used for \Acs{DALB} evaluation}\label{eval_kpi.tab}

      \begin{tabular}{L{0.1\textwidth}L{0.815\textwidth}}      
        \toprule
        \textbf{\Acs{KPI}} & %\textbf{Eval Type} &
        \textbf{Description} \\\midrule
        \Acs{AMST} & 
 \Acl{AMST} (in seconds), i.e., the average delay due to \Acsp{MILP} solution computation\\\hline
 \Acs{MMD} & \Acl{MMD}, i.e., the fraction of \Acsp{MILP} not solved within the $\zeta = 0.5$ mins deadline\\\hline
       \Acs{NHC} & 
 \Acl{NHC}. For user $u$, given $N(u)$ (number of times the adaptive algorithm decided to change the \Acs{MPC} receding horizon) and $T(u)$ (total number of \Acsp{MILP}), then
          \Acs{NHC}$=N(u)/T(u)$
          \\\hline
          \Acs{MPDF} & 
 \Acl{MPDF}. 
          For user $u$, given $R(u)$ (number of times the \Acs{PEV} was plugged) and $M(u)$ (number of times \Acs{EBR} failed to fully re-charge the \Acs{PEV} within the deadline), then
          \Acs{MPDF}$=M(u)/R(u)$
          \\
\hline
          \Acs{LADOBR} & 
 \Acl{LADOBR}, i.e., \Acs{LADOBR}$=1 - \frac{\Delta(e)}{\Delta(d)}$ (see \cref{sec:problem_form}). \\
 \hline
          \Acs{DADOBR} & 
 \Acl{DADOBR}. Let $\Delta(c)$ be the overall aggregated \Ac{DAPP} collaborative profile (see \cref{sec:methodology}) power outside the desired substation bounds. Then, \Acs{DADOBR}$=1 - \frac{\Delta(c)}{\Delta(d)}$. \\            \bottomrule
      \end{tabular}
      \vspace*{-0.5cm}
    \end{table*}

    \newcommand{\Y}{$\bullet$}



    In this section, we describe how we organize our experiments, in order to show the feasibility of our approach. 
    To this aim, we implemented both the \Ac{DAPP} and the \Ac{EBR} algorithm
    by using the Python language, and we use \Ac{GLPK} 
  to solve \Acs{MILP} problems. 
  The following results have been obtained by simulating \Ac{DAPP} operation for one year
  on an Intel i7 2.5 GHz with 8GB of RAM, and
  by simulating \Ac{EBR} operation for the same period, also considering
  output from \Ac{DAPP}, on a Raspberry Pi Model B+ 700 MHz with 512 MB of RAM. 
  Our experiments are organized as follows.

\textbf{\Aclp{KPI}}.
    In order to evaluate our \Ac{DALB} methodology, we define a set of meaningful \Acp{KPI}, which are listed and explained in \cref{eval_kpi.tab}. 

    \begin{figure}
      \vspace*{-0.4cm}
      \IncludeGraphics[width=0.8\columnwidth]{figs/S3.pdf}
      \vspace*{-0.2cm}
      \caption{Net topology of the substation and connected houses}\label{fig:net_top}
    \end{figure}

    \begin{figure}
      \IncludeGraphics[width=1.0\columnwidth,height=0.18\textheight]{figs/stats_houses.pdf}
      \vspace*{-0.1cm}
      \caption{\hl{Houses historical demand distribution}}\label{stats_houses.fig}
      \vspace*{-0.1cm}
    \end{figure}
    
    
    \begin{table}
      \vspace*{0.5cm}
  \centering
  \caption{Parameters for \Acs{DALB} evaluation}\label{exps_params.tab}

  \begin{tabularx}{\linewidth}{llX}    
    \toprule
    \textbf{Param} & \textbf{Value} & \textbf{Explanation}
    \\\hline
    $|U|$ & 62 & Number of houses\\\hline
    $\tau_s$ & 1 day & Gap between two \Ac{MILP} solver invocations for \Ac{DAPP}\\\hline
    $\tau_l$ & 1 hour & Duration of time slots for power limits output by \Ac{DAPP}\\\hline
    $\tau$ & 5 min & Gap between two \Ac{MILP} solver invocations for \Ac{EBR}\\\hline
    $\zeta$ & 30 sec & Deadline for each \Ac{MILP} solver invocation in \Ac{EBR}\\\hline
    $H_i$ & 6 & Starting value for receding horizon in \Ac{EBR}\\\hline
    $H_\delta$ & 7 & Changing step for receding horizon in \Ac{EBR}\\\hline
    $Q_E$ & 13.5 kWh & Battery capacity on each house\\\hline
    $M_E , m_E$ & 3.3 kW & Battery power rate\\\hline
    $\alpha_1 , \beta_1$ & 0.9 & Battery round-trip efficiencies\\\hline
    $Q_P$ & 16 kWh & \Acs{PEV} capacity on each house\\\hline
    $M_P , m_P$ & 3.6 kW & \Acs{PEV} power rate\\\hline
    $\alpha_2 , \beta_2$ & 0.876 & \Acs{PEV} round-trip efficiencies\\
    \bottomrule
  \end{tabularx}
  \vspace*{-0.7cm}
\end{table}

    \textbf{Substation, households and \Acsp{PEV}}.    
    In order to accurately simulate \Ac{DAPP} and \Ac{EBR} operation for a long enough period, we need power demand data, taken at intervals of at least one hour, of each residential house connected to a given substation. To this aim, 
    we use power demand \hl{recorded}, from the beginning of September 2013 to the end of August 2014,
    in 62 households in a suburban area in Denmark. All such houses are connected to the same substation $s$ (see \cref{fig:net_top}). 
    Such data were recorded during the European Commission project ``SmartHG''~\cite{SmartHGweb,Alim2015} and consists, for each of the 62 houses, in the power demand recorded from house electricity main, with a resolution of 1 hour. We point out that Danish households use district heating for house heating and electricity for house appliances.
    We also use \Ac{PVP} energy production recorded in the same period and \hl{area}. Such recorded data consider 6 kWp \Ac{PVP} installations, with highly seasonal productivity ranging from 200 kWh/month in December and above 1200 kWh/month  from April to July.  
    \hl{To assess the validity of our case study,
      we show that, with high probability,
      any operational scenario will be very close to one of those entailed by the houses $U$ considered in our case study.
      To this end, we divide each day into 4 time slots $t_1, \ldots, t_4$ of 6 hours each,
      with $t_i = [6(i - 1), 6i)$ ($i = 1, \ldots, 4$).
        Let $D_u(t_i)$ be the total electricity demand (for a whole year, in our case study) of house $u$ within time slot $t_i$,
        let $D_u^{tot} = \sum_{i = 1}^4 D_u(t_i)$ be the total (whole year) demand of house $u$ and let
        $\tilde{D}_u(t_i)$ be the fraction of the demand of house $u$ within time slot $t_i$,
        i.e., $\tilde{D}_u(t_i) = \frac{D_u(t_i)}{D_u^{tot}}$.
        On such a base, we define the $\emph{demand distribution}$ $\tilde{D}_u$ for house $u$ as $\tilde{D}_u = \left(\tilde{D}_u(t_1), \tilde{D}_u(t_2), \tilde{D}_u(t_3), \tilde{D}_u(t_4)\right)$.
        %
        \mbox{\cref{stats_houses.fig}} shows the set of demand distributions $\tilde{D}$ = $\{\tilde{D}_u \; | \; u \in U\}$.
        Our goal is to show that any \emph{reasonable} demand distribution will not be \emph{too different} from one of those in $\tilde{D}$.
        Accordingly, our set of \emph{admissible} demand distributions is
        $D^{*}$ = $\{(p_1, p_2, p_3, p_4) \; | \; (\land_{i = 1}^4 p_i \in [0.1, 0.3]) \land (\sum_{i = 1}^4 p_i = 1)\}$.
      %
        Given a demand profile $p = (p_1, p_2, p_3, p_4) \in D^{*}$,
        we define the distance $rmse(p)$ of $p$ from $\tilde{D}$ as 
        the minimum root mean square error, i.e.,
        $rmse(p) = \frac{1}{2}\min \left\{\sqrt{\sum_{i = 1}^4 (p_i - \tilde{D}_u(t_i))^2} \;|\; u \in U\right\}$. Note that $rmse(p) = 0$ for $p \in \tilde{D}$. Using MonteCarlo-based statistical model checking techniques (e.g., as in \mbox{\cite{MMMSTGHPE18})}, we can show that, with probability at least 0.99,
        %99.99\%,
        for a randomly selected $p \in D^{*}$ we have $rmse(p) \leq 0.08$. That is, with high probability, any admissible demand distribution will be \emph{very close} to one of those considered in our case study.
        This shows that conclusions drawn from our case study can be safely generalized to other situations.}
    
    Furthermore, 
    we virtually equip each house with \Acp{PEV} charging data taken from the ``Test-an-EV'' project~\cite{SmartHGweb}. Such data consists in plug-in time, \Ac{SOC} at plug-in time and unplug time for 184 \Acp{PEV} Mitsubishi i-MiEV, ranging from 2012 to 2013. The matching between a house and \hl{an} \Ac{PEV} has been done \hl{randomly}. 
    We remark that, in \Ac{DAPP} experiments, \Acp{PEV} charging data is considered a further load for each house $u$, thus the power demand in a time slot $t$ is incremented by the historical charging data of the \Ac{PEV} connected to $u$. In \Ac{EBR} experiments, we only take into account the starting time and starting \Ac{SOC} of each recharge, as well as its unplug time. Then, it is \Ac{EBR} responsibility to decide charge/discharge actions for the \Ac{PEV}.

    \textbf{Substation Bounds}. We split our experiments \hl{into} 3 {\em scenarios}, each corresponding to different values for the desired bounds on substation $s$ required in input by \Ac{DAPP}. In order to set up challenging scenarios for our \Ac{DALB} methodology, we compute, from the historical data on houses power consumption described above (also considering \Ac{PEV} recharging data), the daily average $A(D)$ and daily maximum $M(D)$ on the aggregated power demand, being $D$ a given day. 
    A scenario $S$ is defined by setting, for each day $D$ and all time slots $t$ of $D$, $[P_s^{low}(t), P_s^{high}(t)] = [0, A(D) + S(M(D) - A(D))]$. 
    That is, we set the lower bound to be 0, as reverse power flows may damage any installed electrical equipment in the grid~\cite{DFBS2018}. Instead, for the upper bound, we have that for $S = 0$ it coincides with the daily average, whilst for $S = 1$ it coincides with the daily maximum. The lower $S$, the more challenging our scenario is. In the \hl{following,} we will consider 3 values for $S$, each defining a scenario, i.e., $S \in \{0, 0.25, 0.5\}$.
%


    All other experimental parameters are shown in \cref{exps_params.tab}. Simulation of \Ac{DAPP} 
    in a given day ${\cal D}$ is carried out by taking as input the historical data on power demand of all houses $u \in U$ in day ${\cal D} - 1$, as well as the substation bounds for day ${\cal D}$ as discussed above. For each house $u \in U$, simulation of \Ac{EBR} in time slot $t$ is carried out by taking as input the power limits output by \Ac{DAPP} for $u$ in $T_s$, the power demand of $u$ in $t$ from historical data, and the estimated \Ac{SOC} of battery and \Ac{PEV} in $t$. Such \Ac{SOC} is computed from the \Ac{SOC} and the charge/discharge action of the previous time slot $t-1$, using the first time slot of~\eqref{ess_dyn} and~\eqref{pev_dyn}.

